ImGeoNet: Image-induced Geometry-aware Voxel Representation for Multi-view 3D Object Detection

We propose ImGeoNet, a multi-view image-based 3D object detection framework that models a 3D space by an image-induced geometry-aware voxel representation. Unlike previous methods which aggregate 2D features into 3D voxels without considering geometry, ImGeoNet learns to induce geometry from multi-view images to alleviate the confusion arising from voxels of free space, and during the inference phase, only images from multiple views are required. Besides, a powerful pre-trained 2D feature extractor can be leveraged by our representation, leading to a more robust performance. To evaluate the effectiveness of ImGeoNet, we conduct quantitative and qualitative experiments on three indoor datasets, namely ARKitScenes, ScanNetV2, and ScanNet200. The results demonstrate that ImGeoNet outperforms the current state-of-the-art multi-view image-based method, ImVoxelNet, on all three datasets in terms of detection accuracy. In addition, ImGeoNet shows great data efficiency by achieving results comparable to ImVoxelNet with 100 views while utilizing only 40 views. Furthermore, our studies indicate that our proposed image-induced geometry-aware representation can enable image-based methods to attain superior detection accuracy than the seminal point cloud-based method, VoteNet, in two practical scenarios: (1) scenarios where point clouds are sparse and noisy, such as in ARKitScenes, and (2) scenarios involve diverse object classes, particularly classes of small objects, as in the case in ScanNet200.

==> sections/backup.tex <==

%%%%%%%%% ABSTRACT
\begin{abstract}
   The ABSTRACT is to be in fully-justified italicized text, at the top
   of the left-hand column, below the author and affiliation
   information. Use the word ``Abstract'' as the title, in 12-point
   Times, boldface type, centered relative to the column, initially
   capitalized. The abstract is to be in 10-point, single-spaced type.
   Leave two blank lines after the Abstract, then begin the main text.
   Look at previous ICCV abstracts to get a feel for style and length.
\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the ICCV 2023 web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section,
must be no longer than eight pages in length. The references section
will not be included in the page count, and there is no limit on the
length of the references section. For example, a paper of eight pages
with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for ICCV 2023.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.  

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera-ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the \verb'\iccvfinalcopy' command in the document preamble.)  Reviewers:
note that the ruler measurements do not align well with the lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $095.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future readers
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work --- in fact, it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our
   previous paper [1] and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}

An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the
   paper of Smith \etal [1] and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors14} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a tech report for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors14b}''.  Then submit the tech report as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the ICCV70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead,
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviors
   which shows how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific conventions,
reads better than the first version and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report the results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of a caption.  It is set in Roman so mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.

\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.

Page numbers should be included for review submissions but not for the 
final paper. Review submissions papers should have page numbers in the 
footer with numbers centered and .75 inches (1.905 cm) from the bottom 
of the page and start on the first page with the number 1.

Page numbers will be added by the publisher to all camera-ready papers 
prior to including them in the proceedings and before submitting the 
papers to IEEE Xplore. As such, your camera-ready submission should 
not include any page numbers. Page numbers should automatically be 
removed by uncommenting (if it's not already) the line
\begin{verbatim}
% \iccvfinalcopy
\end{verbatim}
near the beginning of the .tex file.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centered.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths that render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}

%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the ICCV 2023 web page for a discussion
of the use of color in your document.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.


==> sections/experiment/result/eval_metric.tex <==
  \mdsubsec{Evaluation Metric.}
  We adopt mean average precision (mAP) to evaluate the detection accuracy.
  Specifically, we use mAP@0.25 and mAP@0.5 where the numbers indicate the 3D intersection over union (IoU) thresholds.
  To explain, the threshold is the minimum IoU to determine a positive match, which makes mAP@0.5 be more strict on the object location evaluation than mAP@0.25.~\yulunliu{Can we move these detail to section 4.1 titled: Experimental setup? And put the dataset, metric, and compared methods as three subsections in 4.1.}

==> tables/v1/ablation_geo_shaping.tex <==
\begin{table}[t!]
\small
\centering
\caption{
  \textbf{Effectiveness of the geometry shaping}.
  Despite the fact that ImVoxelNet with state-of-the-art multi-view depth estimator, MaGNet, (j-2) takes 5 times more input views and has a larger model size and a much longer runtime, {\ourmethod} has better detection result on ScanNetV2.
  The model size and the inference time of {\ourmethod} on ScanNetV2 is 485.6 MB and 489.9 ms, respectively.
  The experiment is run by a single GTX-3090 GPU and the data loading time is ignored.
  \vspace{5pt}
}
\begin{tabular}{l|c|c|cc}
    \toprule
     & \multicolumn{2}{c|}{Relative} & \multicolumn{2}{c}{mAP} \\
    \cmidrule(lr){2-5}
    Method & Size & Runtime & @0.25 & @0.5 \\
    \midrule
    (j-1) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & 0.82 & 0.85 & 48.7 & 23.8 \\
    (j-2) ~~w/ MaGNet~\cite{bae2022magnet} & 1.42 & 15.72 & 53.8 & 28.2 \\
    (j-3) ~~w/ GT depth & 0.82 & 0.89 & 58.8 & 33.4 \\
    \midrule
    (k-1) {\ourmethod} (ours) & 1.0 & 1.0 & \textbf{54.8} & \textbf{28.4} \\
    \bottomrule \addlinespace
\end{tabular}
\label{table:scannet-ablation-geo-shaping}
\end{table}


==> tables/v1/main_arkit.tex <==
\begin{table*}[ht!]
\small
\centering
\caption{
  \textbf{3D object detection result on ARKitScenes}.
  To show the feasibility of the proposed method in realistic scenes, we present the detection results on ARKitScenes with different number of input views.
  We emphasize that our method with only 40 views can reach the performance of ImVoxelNet with 100 views.
  \vspace{5pt}
}
\begin{tabular}{l|c|c|c|c|c|c|c}
    \toprule
    & \multicolumn{7}{c}{Performance (mAP@0.25/mAP@0.5)} \\
    \cmidrule(lr){2-8}
    Method & 10 views & 20 views & 30 views & 40 views & 50 views & 75 views & 100 views\\
    \midrule
    (f-1) VoteNet~\cite{qi2019votenet} & 30.2 / 20.8 & 45.9 / 31.5 & 50.2 / 34.0 & 51.1 / 36.8 & 53.3 / 38.5 & 53.6 / 38.3 & 53.9 / 39.0\\
    (f-2) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & 36.2 / 19.6 & 50.5 / 30.6 & 54.6 / 35.2 & 57.4 / 37.9 & 58.0 / 38.8 & 58.8 / 40.5 & 59.7 / 42.0\\
    % (f-3)  ~~w/ GT depth & - & - & - & - & 62.2 / 46.4 & - & -\\
    \midrule
    (g-1) {\ourmethod} (ours) & \textbf{39.0} / \textbf{21.9} & \textbf{53.1} / \textbf{34.3} & \textbf{57.1} / \textbf{39.2} & \textbf{59.5} / \textbf{42.7} & \textbf{60.2} / \textbf{43.4} & \textbf{61.8} / \textbf{45.0} & \textbf{62.4} / \textbf{45.7}\\
    \bottomrule \addlinespace
\end{tabular}
\label{table:arkit-result}
\end{table*}


==> tables/v1/main_scannet.tex <==
\begin{table}[ht!]
\small
\centering
\caption{
  \textbf{3D object detection result on ScanNetV2}.
  {\ourmethod} surpasses the image-based state-of-the-art method, ImVoxelNet,  by a notable margin.
  Besides, the performance of {\ourmethod} with 50 views is close to the point cloud based baseline, VoteNet, even though VoteNet leverages reconstructed meshes derived from multiple viewpoints, typically consisting of more than 1000 views, to obtain high-quality point clouds for its operations.
  RGB and PC fields indicate the input modality for each method.
}
\vspace{5pt}
\begin{tabular}{l|cc|cc}
    \toprule
     & \multicolumn{2}{c|}{Input} & \multicolumn{2}{c}{Performance (mAP)} \\
    \cmidrule(lr){2-5}
    Method & RGB & PC & @0.25 & @0.5 \\
    \midrule
    (a-1) VoteNet~\cite{qi2019votenet} & - & \checkmark & \textbf{58.6} & \textbf{33.5} \\
    (a-2) 3D-SIS~\cite{hou20193dsis} & - & \checkmark & 25.4 & 14.6 \\
    (a-3) 3D-SIS~\cite{hou20193dsis} & \checkmark & \checkmark & 40.2 & 22.5 \\
    %(a-4) H3DNet~\cite{zhang2020h3dnet} & - & \checkmark & 67.2 & 48.1 \\
    \midrule
    (b-1) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & \checkmark & - & 48.7 & 23.8 \\
    \midrule
    (c-1) {\ourmethod} (ours) & \checkmark & - & 54.8 & 28.4 \\
    \bottomrule \addlinespace
\end{tabular}
\label{table:scannet-result}
\end{table}


==> tables/v1/main_scannet200.tex <==
\begin{table*}[ht!]
\small
\centering
\caption{
  \textbf{3D object detection result on ScanNet200}.
  To examine the robustness of the proposed method for diverse classes, we evaluate our method on ScanNet200.
  As in the official benchmark, we group categories into head, common and tail groups where the average object sizes decrease from the head to the tail group.
  RGB and PC fields indicate the input modality for each method.
  \vspace{5pt}
}
\begin{tabular}{l|cc|cc|cc|cc|cc}
    \toprule
     & & & \multicolumn{8}{c}{Performance (mAP)} \\
    \cmidrule(lr){4-11}
     & \multicolumn{2}{c|}{Input} & \multicolumn{2}{c|}{Head} & \multicolumn{2}{c|}{Common} & \multicolumn{2}{c|}{Tail} & \multicolumn{2}{c}{Total} \\
    \cmidrule(lr){2-11}
    Method & RGB & PC & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5 \\
    \midrule
    (d-1) VoteNet~\cite{qi2019votenet} & - & \checkmark & \textbf{38.5} & \textbf{20.0} & 16.0 & \textbf{8.0} & 2.9 & 1.8 & 19.8 & \textbf{10.3} \\
    (d-2) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & \checkmark & - & 34.1 & 15.2 & 14.0 & 4.2 & 7.7 & \textbf{2.3} & 19.0 & 7.4 \\
    \midrule
    (e-1) {\ourmethod} (ours) & \checkmark & - & 38.1 & 18.7 & \textbf{17.3} & 6.9 & \textbf{9.7} & 1.5 & \textbf{22.3} & 9.4 \\
    \bottomrule \addlinespace
\end{tabular}
\label{table:scannet200-result}
\end{table*}


==> tables/v1/speed.tex <==
\begin{table*}[ht!]
\small
\centering
\caption{
  \textbf{Inference time for 3D object detection}.
  Different numbers of views are provided for runtime evaluation.
  The experiment is run on ARKitScenes with a single GTX-3090 GPU.
  The data loading time is ignored and the inference times are averaged over all test scenes.
  \vspace{5pt}
}
\begin{tabular}{l|c|c|c|c|c|c|c}
    \toprule
    & \multicolumn{7}{c}{Inference Time (millisecond)} \\
    \cmidrule(lr){2-8}
    Method & 10 views & 20 views & 30 views & 40 views & 50 views & 75 views & 100 views\\
    \midrule
    (t-1) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & 97.3 & 113.1 & 126.5 & 140.0 & 155.9 & 188.2 & 219.7\\
    \midrule
    (t-2) {\ourmethod} (ours) & 122.5 & 139.0 & 152.4 & 166.1 & 181.8 & 214.1 & 245.8\\
    \bottomrule \addlinespace
\end{tabular}
\label{table:speed}
\end{table*}


==> tables/v2/comp_scannet200.tex <==
\begin{table*}[ht!]
\small
\centering
\caption{
  \textbf{3D object detection results on ScanNet200}.
  To examine the robustness of the proposed method for diverse classes, we evaluate our method on ScanNet200.
  As in the official benchmark, we group categories into head, common and tail groups where the average object sizes decrease from the head to the tail group.
  The notations RGB and PC signify the utilization of color image and point cloud in the process of inference, respectively.
  \vspace{5pt}
}
\begin{tabular}{l|cc|cc|cc|cc|cc}
    \toprule
     & & & \multicolumn{8}{c}{Performance (mAP)} \\
    \cmidrule(lr){4-11}
     & \multicolumn{2}{c|}{Input} & \multicolumn{2}{c|}{Total} & \multicolumn{2}{c|}{Head} & \multicolumn{2}{c|}{Common} & \multicolumn{2}{c}{Tail} \\
    \cmidrule(lr){2-11}
    Method & RGB & PC & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5 \\
    \midrule
    (d-1) VoteNet~\cite{qi2019votenet} & - & \checkmark & 19.8 & \textbf{10.3} & \textbf{38.5} & \textbf{20.0} & 16.0 & \textbf{8.0} & 2.9 & 1.8 \\
    \midrule
    (d-2) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & \checkmark & - & 19.0 & 7.4 & 34.1 & 15.2 & 14.0 & 4.2 & 7.7 & \textbf{2.3} \\
    (d-3) {\ourmethod} (ours) & \checkmark & - & \textbf{22.3} & 9.4 & 38.1 & 18.7 & \textbf{17.3} & 6.9 & \textbf{9.7} & 1.5 \\
    \bottomrule \addlinespace
\end{tabular}
\label{table:scannet200-result}
\end{table*}


==> tables/v2/nouse_img_comp.tex <==
\begin{table}[ht!]
\small
\centering
\caption{
  \textbf{Comparison with the state-of-the-art image-based method}. {\ourmethod} surpasses the state-of-the-art image-based method, ImVoxelNet, by a notable margin on all three datasets.
  For each dataset, we evenly sample 50 views from each scene for training or testing.
}
\vspace{5pt}
\begin{tabular}{l|c|c|c}
    \toprule
     & \multicolumn{3}{c}{Performance (mAP@0.25 / mAP@0.5)} \\
    \cmidrule(lr){2-4}
    Method & ARKitScenes & ScanNetV2 & ScanNet200 \\
    \midrule
    ImVoxelNet~\cite{rukhovich2022imvoxelnet} & 58.0 / 38.8 & 48.7 / 23.8 & 19.0 / 7.4 \\
    % \midrule
    {\ourmethod} (ours) & \textbf{60.2} / \textbf{43.4} & \textbf{54.8} / \textbf{28.4} & \textbf{22.3} / \textbf{9.4} \\
    \bottomrule \addlinespace
\end{tabular}
\label{table:img-based-comparison}
\end{table}


==> tables/v2/nouse_pcd_comp.tex <==
\begin{table*}[ht!]
\small
\centering
\caption{
  \textbf{Comparison with point cloud based baselines}.
}
\vspace{5pt}
\begin{tabular}{l|cc|c|c|c|c|c|c}
    \toprule
    & & & \multicolumn{6}{c}{Performance (mAP@0.25 / mAP@0.5)} \\
    \cmidrule(lr){4-9}
     & \multicolumn{2}{c|}{Input} & ARKitScenes & ScanNetV2 & \multicolumn{4}{c}{ScanNet200} \\
    \cmidrule(lr){2-9}
    Method & RGB & PC & Total & Total & Head & Common & Tail & Total \\
    \midrule
    % Method & RGB & PC & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5 \\
    % \midrule
    3D-SIS~\cite{hou20193dsis} & - & \checkmark & - & 25.4 / 14.6 & - & - & - & - \\
    3D-SIS~\cite{hou20193dsis} & \checkmark & \checkmark & - & 40.2 / 22.5 & - & - & - & - \\
    VoteNet~\cite{qi2019votenet} & - & \checkmark & 53.3 / 38.5 & \textbf{58.6} / \textbf{33.5} & \textbf{38.5} / \textbf{20.0} & 16.0 / \textbf{8.0} & 2.9 / 1.8 & 19.8 / \textbf{10.3} \\
    \midrule
    ImVoxelNet~\cite{rukhovich2022imvoxelnet} & \checkmark & - & 58.0 / 38.8 & 48.7 / 23.8 & 34.1 / 15.2 & 14.0 / 4.2 & 7.7 / \textbf{2.3} & 19.0 / 7.4 \\
    % \midrule
    {\ourmethod} (ours) & \checkmark & - & \textbf{60.2} / \textbf{43.4} & 54.8 / 28.4 & 38.1 / 18.7 & \textbf{17.3} / 6.9 & \textbf{9.7} / 1.5 & \textbf{22.3} / 9.4 \\
    % ImVoxelNet~\cite{rukhovich2022imvoxelnet} & \checkmark & - & 34.1 & 15.2 & 14.0 & 4.2 & 7.7 & \textbf{2.3} & 19.0 & 7.4 \\
    % \midrule
    % {\ourmethod} (ours) & \checkmark & - & 38.1 & 18.7 & \textbf{17.3} & 6.9 & \textbf{9.7} & 1.5 & \textbf{22.3} & 9.4 \\
    \bottomrule \addlinespace
\end{tabular}
\label{table:scannet200-result}
\end{table*}


==> tables/v2/nouse_speed_all.tex <==
\begin{table*}[ht!]
\small
\centering
\caption{
  \textbf{Inference time for 3D object detection}.
  Different numbers of views are provided for runtime evaluation.
  The experiment is run on ARKitScenes with a single GTX-3090 GPU.
  The data loading time is ignored and the inference times are averaged over all test scenes.
  \vspace{5pt}
}
\begin{tabular}{l|c|c|c|c|c|c|c}
    \toprule
    & \multicolumn{7}{c}{Inference Time (millisecond)} \\
    \cmidrule(lr){2-8}
    Method & 10 views & 20 views & 30 views & 40 views & 50 views & 75 views & 100 views\\
    \midrule
    (t-1) ImVoxelNet~\cite{rukhovich2022imvoxelnet} & 97.3 & 113.1 & 126.5 & 140.0 & 155.9 & 188.2 & 219.7\\
    \midrule
    (t-2) {\ourmethod} (ours) & 122.5 & 139.0 & 152.4 & 166.1 & 181.8 & 214.1 & 245.8\\
    \bottomrule \addlinespace
\end{tabular}
\label{table:speed}
\end{table*}

